Smart PRACH Jamming: A Serious Threat for 5G Campus Networks

Smart jamming attacks on cellular campus networks represent an enormous potential threat, especially in the industrial environment. In complex production processes, the disruption of a single wireless connected Cyber-Physical System (CPS) is enough to cause a large-scale failure. In this paper, a smart jamming attack on the Physical Random Access Channel (PRACH) of a 5G system is modeled. This is followed by a practical implementation of the jammer on a testbed based on Open Air Interface (OAI) and Software Defined Radios (SDRs). It is shown that the designed jammer design can interfere a legitimate transmission of a PRACH preamble with a ratio of more than 99.9%. While less than one percent of the cell resources are interfered compared to broadband jamming. In addition, two different types of jamming signal spectra are compared in relation to their interference capacity. The developed attack can be re-implemented based on publicly available source code and Commercial Off-The-Shelf (COTS) hardware.

==> 1supply/glossaries_JuSt.tex <==
%________________________________________________________________________
%------------------------------------------------------------------------
%       Package Extensions are performed in files
% - - - - - - - - - - - - -
%           "0organization/1main/3settings/4customization/glossaries_keys.tex"
%           "0organization/1main/3settings/4customization/glossaries_cmds.tex"
%       This supplies an additional Glossary-Entry-Creation Makro for simultaneously filling in an Acronym and corresponding Glossary-Entry, being referenced. (Usage see later below)
%       Also additional "Custom Keys" are defined to extend Entries with more values
%           The Custom Keys are
%               deutsch, englisch, untertitel, alternativ, url, longpltwo
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%------------------------------------------------------------------------
%________________________________________________________________________
%
%
%
%
%
%________________________________________________________________________
%------------------------------------------------------------------------
%				Central Terms of this Document (aka Thesis, Paper, Letter, ...)
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
% \newglossaryentry{denkrsuite}{%
% 	name={DenKr\_Suite},%
% 	description={A collective term for all elements of the software solution provided by this Thesis.},%
% }%
% \newdualentry%
% []% Options für Glossary
% []% Options für Acronym
% {archd}% label
% {ArchDaemon}% abbreviation
% {Architecture-Daemon}% long form
% {Part of the \gls{denkrsuite}. \textit{\gls{integhierarchl}~4} of the \gls{integhierarch} from the \gls{denkrnuc}.}% description
% % % % % % % % % % % % % % %
% \newacronym{Key}{Abbreviation}{WrittenOut}%
% \glsunset{Key}%
%
%
%
%------------------------------------------------------------------------
%				Former Documents
%========================================================================
\newacronym{ar}{AR}{Application Relation}%
\newacronym{indeco}{InDeCo}{Interconnection Detachment \& Convergence}%ArchDaemon-Tool: Interconnection
\newacronym{coma}{CoMa}{Context-Management}%ArchDaemon-Tool: Context-Management
\newacronym{peac}{PeAc}{Permission \& Access}%ArchDaemon-Tool: Permission & Access
\newacronym{dynploy}{DynPloy}{Dynamic Deployment}%ArchDaemon-Tool: Dynamic Deployment
\newacronym{remcon}{RemCon}{Remote Configuration}%ArchDaemon-Tool: Device \& Service Remote Configuration
\newacronym{coagd}{CAD}{Collective Aggregator Discovery}%DenKrement-Tool: Automatic Self-Organizing Network Device Discovery  (Operates sparsam, kollaborativ)  ("Capacity-aware/Economical, Collaborative Network Device Discovery")
\newacronym{archdaemon}{ArchDaemon}{Architecture-Daemon}
\newacronym{ctrllog}{ACL}{Aggregated Control Logic}
\newacronym{adagent}{ADAg}{ArchDaemon-Agent}
\newacronym{adaloc}{ADAl}{ArchDaemon-Allocator}%Commissioner, Allocator, Controller, Hub, Pivot
\newacronym{inserv}{InServ}{Inserted-Service}% Inserted/Infrastrucure Service  |  service, item, component,
\newacronym{infrserv}{InfrServ}{Infrastructure-Service}% unit, member, extension, addition, attachment, additive
\newacronym{atserv}{AtServ}{Atop-Service}%
\newacronym{orcus}{OrCuS}{Organic Customization System}% Culmination, Cumulation
\newacronym{ore}{ORE}{Organic Runtime Environment}%
\newacronym{relag}{Agent}{Agent}%
\newacronym{relorc}{Orc}{Orchestrator}%
\newacronym{slaag}{SLAAg}{Service Level Agreement Agent}%
\newacronym{cmdc}{CMDC}{Centralized Mission and Driving Control}%
\newacronym{dcmod}{DCMod}{Data Collection Module}%
\newacronym{posmod}{PosMod}{Positioning Module}%
\newacronym{mts}{MTS}{Map Transformation Stage}%
\newacronym{sensmod}{SensMod}{Sensing Module}%
\newacronym{sidr}{SIDR}{Sensor ID Resolver}%
\newacronym{camod}{CAMod}{Carrier Aggregation Module}%
\newacronym{muxs}{MuxS}{Multiplexer Stage}%
\newacronym[plural=CSEs,%
	firstplural=Carrier State Estimators (CSEs),%
	longplural=Carrier State Estimators]%
	{cse}{CSE}{Carrier State Estimator}%
\newacronym{ca}{CA}{Carrier Aggregator}%
\newacronym[plural=IAs,%
	firstplural=Information Anchors (IAs),%
	longplural=Information Anchors]%
	{ia}{IA}{Information Anchor}%
\newacronym{dbmod}{DBMod}{Data Base Module}%
\newacronym{bui}{BUI}{Base User Interface}%
\newacronym{bman}{BMan}{Base Manager}%
\newacronym[plural=DSs,%
	firstplural=Data Suppliers (DSs),%
	longplural=Data Suppliers]%
	{ds}{DS}{Data Supplier}%
\newacronym[plural=GWs,%
	firstplural=Gateways (GWs),%
	longplural=Gateways]%
	{gw}{GW}{Gateway}%
\newacronym{auditf}{TTF}{Trust \& Traceability Function}%
\newacronym{specal}{SASF}{Spectrum Allocation \& Sharing Function}%
%------------------------------------------------------------------------
%________________________________________________________________________
%
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%					Central Terms done
%------------------------------------------------------------------------
%________________________________________________________________________
%
%
%
%
%
%________________________________________________________________________
%------------------------------------------------------------------------
%						Glossar
%  -  -  -  -  -  -  -
% Example:
%        \newglossaryentry{trunking}{%
%        	name={Trunking},%
%        	text={Trunking},%
%        	deutsch={Bündelung},%
%        	untertitel={Datenübertragung},%
%        	alternativ={Link Aggregation},%
%        	description={\label{gls:trunking}%
%                In der Nachrichtentechnik und Informatik bezeichnet >>Trunking<< [...]%
%           },%
%        }
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\

%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%						Glossar fertig
%------------------------------------------------------------------------
%________________________________________________________________________
%
%
%
%
%
%________________________________________________________________________
%------------------------------------------------------------------------
%						Akronyme (Abkürzungen)
%                       -- (More Universal) --
%  -  -  -  -  -  -  -
% Example:
%        \newacronym{sdning}{SDN}{Software-Defined Networking}%
%        \newacronym[plural=SDNs,%
%        	firstplural=Software-Defined Networks (SDNs),%
%        	longplural=Software-Defined Networks]%
%        	{sdn}{SDN}{Software-Defined Network}%
%        \glsunset{sdn}%
%        \newacronym[see={[Glossar:]{gls-endTE}}]{endTEde}{ETE}{Ende-zu-Ende}%Don't create such an acronym entry explicitly if you use the supplied dualentry-cmd below
%        \newacronym[englisch=Virtual Machine,%
%        	plural=VMs,%
%        	firstplural=Virtuelle Maschinen (VMs),%
%        	longplural=Virtuelle Maschinen]%
%        {vm}{VM}{Virtuelle Maschine}%
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%
%--------------------------------------------------------
% = = = General Terms
%________________________________________________________
\newacronym{example}{e.g.}{exempli gratia}
\newacronym{qos}{QoS}{Quality-of-Service}%
\glsunset{qos}%
\newacronym{utc}{UTC}{Coordinated Universal Time}%
\newacronym[plural=KPIs,%
	firstplural=Key Performance Indicators (KPIs),%
	longplural=Key Performance Indicators]%
	{kpi}{KPI}{Key Performance Indicator}%
\newacronym{poc}{PoC}{Proof-of-Concept}%
\newacronym{wip}{WiP}{Work in Progress}%
%--------------------------------------------------------
% = = = Specific for: IT, Basic Technology
%________________________________________________________
\newacronym{inft}{IT}{Information Technology}%
\newacronym{fsm}{FSM}{Finite-State Machine}%
\newacronym{fsa}{FSA}{Finite-State Automaton}%
\newacronym[longplural={Distributed Ledger Technologies}]{dlt}{DLT}{Distributed Ledger Technology}%
\newacronym{gps}{GPS}{Global Positioning System}%
\newacronym{trl}{TRL}{Technology Readiness Level}%
\newacronym{opsys}{OS}{Operating System}%
\newacronym{digt}{DT}{Digital Twin}%
%--------------------------------------------------------
% = = = Specific for: Research (i.e. no one in the practical, operating, real word out there uses such stuff)
%________________________________________________________
\newacronym{rand}{R\&D}{Research \& Development}%
\newacronym{softdr}{SDR}{Software Defined Radio}%
%--------------------------------------------------------
% = = = Specific for: Software, Design, Architecture, Paradigm, Development, DevOps, CI/CD
%________________________________________________________
\newacronym{api}{API}{Application Programming Interface}%
\newacronym{uri}{URI}{Uniform Resource Identifier}%
\newacronym{netfunc}{NF}{Network Function}%
\newacronym{nfv}{NFV}{Network Function Virtualization}%
\newacronym{typlv}{TLV}{Type-Length-Value}%
\newacronym{loc}{LoC}{Lines of Code}%
%--------------------------------------------------------
% = = = Specific for: Network Communication, Distributed Systems
%________________________________________________________
\newacronym{url}{URL}{Uniform Resource Locator}%
\newacronym{nic}{NIC}{Network Interface Card}%
\newacronym{rest}{REST}{Representational State Transfer}%
\newacronym{ftp}{FTP}{File Transfer Protocol}%
\newacronym{http}{HTTP}{Hypertext Transfer Protocol}%
\newacronym{https}{HTTPS}{Hypertext Transfer Protocol Secure}%
\newacronym{rpc}{RPC}{Remote Procedure Call}%
\newacronym{lldp}{LLDP}{Link Layer Discovery Protocol}%
\newacronym{snmp}{SNMP}{Simple Network Management Protocol}%
\newacronym{nsh}{NSH}{Network Service Header}%
\newacronym{sdn}{SDN}{Software-defined Networking}%
%\glsunset{sdn}%
\newacronym[plural=SDNs,%
	firstplural=Software-defined Networks (SDNs),%
	longplural=Software-defined Networks]%
	{sdnet}{SDN}{Software-defined Network}%
\newacronym{ip}{IP}{Internet Protocol}%
\glsunset{ip}%
\newacronym{tcp}{TCP}{Transmission Control Protocol}%
\newacronym{udp}{UDP}{User Datagram Protocol}%
\newacronym{dns}{DNS}{Domain Name System}%
\newacronym{ntp}{NTP}{Network Time Protocol}%
\newacronym{ptp}{PTP}{Precision Time Protocol}%
\newacronym{p2p}{P2P}{Point-to-Point}%
\newacronym{peer2p}{Peer2P}{Peer-to-Peer}%
\newacronym{m2m}{M2M}{Machine-to-Machine}%
\newacronym{rbs}{RBS}{Reference Broadcast Time Synchronization}%
\newacronym{rbis}{RBIS}{Reference Broadcast Infrastructure Synchronization}%
\newacronym{mdns}{mDNS}{Multicast DNS}%
\newacronym{dnssd}{DNS-SD}{DNS Service Discovery}%
\newacronym{servoa}{SOA}{Service-Oriented Architecture}%
\newacronym{rtt}{RTT}{Round Trip Time}%
\newacronym{csp}{CSP}{Communication Service Provider}%
\newacronym{mmtc}{MMTC}{Massive Machine Type Communication}%
\newacronym{arq}{ARQ}{Automatic Repeat Request}%
\newacronym{ppm}{PPM}{Parallel Process Migration}%
\newacronym{checkres}{C/R}{Checkpoint/Restore}%
%--------------------------------------------------------
% = = = Specific for: Wireless Communication, Radio
%________________________________________________________
\newacronym{snr}{SNR}{Signal to Noise Ratio}%
\newacronym{acp}{AP}{Access-Point}%
\newacronym{urllc}{URLLC}{Ultra Reliable Low Latency Communication}%
\newacronym{bnetza}{BNetzA}{Bundesnetzagentur}%
%--------------------------------------------------------
% = = = Specific for: Mobile Communications, 5G, 6G
%________________________________________________________
\newacronym{5gsba}{SBA}{5G Service Based Architecture}%
\newacronym{sba}{SBA}{Service Based Architecture}%
\newacronym{mano}{MANO}{Management \& Orchestration}%
\newacronym{ran}{RAN}{Radio Access Network}%
\newacronym{cran}{C-RAN}{Centralized - Radio Access Network}%
\newacronym{oran}{O-RAN}{Open - Radio Access Network}%
\newacronym{sbi}{SBI}{Service Based Interface}%
\newacronym{jcas}{JC\&S}{Joint Communication and Sensing}%
\newacronym{rrm}{RRM}{Radio Resource Management}%
\newacronym{uequ}{UE}{User Equipment}%
\newacronym{gmlc}{GMLC}{Gateway Mobile Location Center}%
\newacronym{embb}{eMBB}{enhanced Mobile Broad-band}%
\newacronym{mnoper}{MNO}{Mobile Network Operator}%
\newacronym{coretc}{CtC}{Core-to-Core}%
\newacronym{gnodb}{gNB}{5G gNodeB Basestation}%
\newacronym{3gpp}{3GPP}{3rd Generation Partnership Project}%
\newacronym{uwb}{UWB}{Ultra Wideband}%
\newacronym{newr}{NR}{New Radio}%
\newacronym{runit}{RU}{Radio Unit}%
\newacronym{cunit}{CU}{Centralized Unit}%
\newacronym{dunit}{DU}{Distributed Unit}%
\newacronym{cpl}{CP}{Control Plane}%
\newacronym{upl}{UP}{User Plane}%
%  -  - Core Functions
\newacronym{ngap}{NGAP}{Next Generation Application Protocol}%
\newacronym{amf}{AMF}{Access and Mobility Management Function}%
\newacronym{lmf}{LMF}{Localization Management Function}%
\newacronym{nef}{NEF}{Network Exposure Function}%
\newacronym{nrf}{NRF}{Network Repository Function}%
\newacronym{scp}{SCP}{Service Communication Proxy}%
%--------------------------------------------------------
% = = = Specific for: Industry, Industrial Communication, Industry 4.0
%________________________________________________________
\newacronym{i40}{I4.0}{Industry 4.0}%
\newacronym{plc}{PLC}{Programmable Logic Controller}%
\newacronym{vpc}{VPC}{Virtual Process Controller}%
\newacronym{tsn}{TSN}{Time-Sensitive Networking}%
\newacronym{cnc}{CNC}{Central Network Controller}%
\newacronym{cuc}{CUC}{Central User Configuration}%
\newacronym{tsncnc}{TSN CNC}{TSN Central Network Controller}%
\newacronym{tssdn}{TSSDN}{Time-Sensitive Software-Defined Networking}%
\newacronym{cpci}{CPCI}{Central Process Control Instance}%
\newacronym{optech}{OT}{Operation Technology}%
%--------------------------------------------------------
% = = = Specific for: Automation, Robotic, Logistics
%________________________________________________________
\newacronym{iot}{IoT}{Internet of Things}%
\newacronym{iiot}{IIoT}{Industrial Internet of Things}%
\newacronym{agv}{AGV}{Automated Guided Vehicle}%
\newacronym{amr}{AMR}{Autonomous Mobile Robot}%
\newacronym{uav}{UAV}{Unmanned Aerial Vehicle}%
\newacronym{erp}{ERP}{Enterprise Resource Planning}%
\newacronym{ips}{IPS}{Indoor Positioning System}%
\newacronym{vmc}{VMC}{Vehicle Motion Control}%
\newacronym{imu}{IMU}{Inertial Measurement Unit}%
\newacronym{ros}{ROS}{Robot Operating System}%
\newacronym{opc}{OPC}{Open Platform Communication}%
\newacronym{opcua}{\gls{opc} UA}{OPC Unified Architecture}%
\newacronym{mqtt}{MQTT}{Message Queue Telemetry Transport}%
\newacronym{etl}{ETL}{Extract, Transfer, Load}%
\newacronym{dds}{DDS}{Data Distribution Service}%
% = = = Localization
\newacronym{dgps}{DGPS}{Differential Global Positioning System}%
\newacronym{ecef}{ECEF}{Earth-centered, Earth-fixed}%
\newacronym{gnss}{GNSS}{Global Navigation Satellite System}%
%--------------------------------------------------------
% = = = Specific for: Artificial Intelligence (AI), Künstliche Intelligenz (KI)
%________________________________________________________
\newacronym{arti}{AI}{Artificial Intelligence}%
\newacronym{mlearn}{ML}{Machine Learning}%
\newacronym{svm}{SVM}{Support Vector Machine}%
%--------------------------------------------------------
% = = = Specific for: Business
%________________________________________________________
\newacronym{sla}{SLA}{Service Level Agreement}%
\newacronym{b2b}{B2B}{Business-To-Business}%
\newacronym{b2c}{B2C}{Business-To-Consumer}%
\newacronym{pmse}{PMSE}{Programme Making and Special Events}%
\newacronym{ppdr}{PPDR}{Public Protection and Disaster Relief}%
%--------------------------------------------------------
% = = = Own glossaries
\newacronym{cps}{CPS}{Cyber-Physical System}
\newacronym{prach}{PRACH}{Physical Random Access Channel}
\newacronym{pbch}{PBCH}{Physical Broadcast Channel}
\newacronym{pdcch}{PDCCH}{Physical Downlink Control Channel}
\newacronym{pucch}{PUCCH}{Physical Uplink Control Channel}
\newacronym{pdsch}{PDSCH}{Physical Downlink Shared Channel}
\newacronym{pusch}{PUSCH}{Physical Uplink Shared Channel}
\newacronym{fr}{FR}{Frequency Range}
\newacronym{oai}{OAI}{Open Air Interface}
\newacronym{tdd}{TDD}{Time Division Duplexing}
\newacronym{cots}{COTS}{Commercial Off-The-Shelf}
\newacronym{ber}{BER}{Bit Error Rate}
\newacronym{ra}{RA}{Random Access}
\newacronym{stal}{SA}{Stand Alone}
\newacronym{rrc}{RRC}{Radio Ressource Control}
\newacronym{rar}{RAR}{Random Access Response}
\newacronym{cpr}{CP}{Cyclic Prefix}
\newacronym{rel}{RE}{Resource Element}
\newacronym{prb}{PRB}{Physical Resource Block}
\newacronym{sfn}{SFN}{System Frame Number}
\newacronym{mnc}{MNC}{Mobile Network Code}
\newacronym{mcc}{MCC}{Mobile Country Code}
\newacronym{mib}{MIB}{Master Information Block}
\newacronym{sib}{SIB}{System Information Block}
\newacronym{ofdm}{OFDM}{Orthogonal Frequency-Division Multiplexing}
\newacronym{phy}{PHY}{Physical}
\newacronym{fft}{FFT}{Fast Fourier Transformation}
\newacronym{ifft}{IFFT}{Inverse Fast Fourier Transformation}
\newacronym{soc}{SoC}{System-on-a-Chip}
\newacronym{siso}{SISO}{Single Input Single Output}
\newacronym{mimo}{MIMO}{Multiple Input Multiple Output}
\newacronym{usrp}{USRP}{Universal Software Radio Peripheral}
\newacronym{dos}{DoS}{Denial of Service}
\newacronym{ris}{RIS}{Reconfigurable Intelligent Surfaces}
\newacronym{pps}{PPS}{Pulse Per Second}

%________________________________________________________
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%						Akronyme fertig
%------------------------------------------------------------------------
%________________________________________________________________________
%
%
%
%
%
%
%________________________________________________________________________
%------------------------------------------------------------------------
%						Dual Entrys
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
% Usage Syntax:
% \newdualentry[glossary options][acronym options]{label}{abbrv}{long}{description}
% and for the references:
% Refer to acronym with \gls{label} and the glossary with \gls{gls-label}
%  -  -  -  -  -  -  -
% Example:
%        \newdualentry%
%        [%
%            deutsch={Programmierschnittstelle},%
%            parent={},%
%            untertitel={}%
%        ]%Options für Glossary
%        [%
%            plural=APIs,%
%            longplural=Programmierschnittstellen%
%        ]%Options für Acronym
%        {api}%label
%        {API}%abbreviation
%        {Application Programming Interface}%long form
%        {%//%
%            Eine \textit{Schnittstelle zur Anwendungsprogrammierung} [...]]%
%        }%description
%        \glsunset{api}%
% Blank Boilerplate:
%\newdualentry%
%[]% Options für Glossary
%[]% Options für Acronym
%{lbl}% label
%{abbr}% abbreviation
%{longf}% long form
%{desc}% description
%________________________________________________________________________
%						Dual Entry Definitions
%VVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVV

%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%						Dual Entrys fertig
%-------------------------------------------------------------------------
%_________________________________________________________________________
%

==> organization/IEEE_authors.tex <==
% author names and affiliations
% use a multiple column layout for up to three different
% affiliations
\author{%
%
\IEEEauthorblockN{%
    Michael Gundall\IEEEauthorrefmark{1},\\%
    %Christoph Fischer\IEEEauthorrefmark{2}%
}
\IEEEauthorblockA{%
    German Research Center for\\Artificial Intelligence GmbH, DFKI\\%
    Trippstadter Str. 122\\%
    67663 Kaiserslautern\\%
    Email: %{\tt
      \{%
        \IEEEauthorrefmark{1}dennis.krummacker,\\%
        \hspace*{1em}\IEEEauthorrefmark{2}christoph.fischer%
      \}@dfki.de
    %}%
}
%
\and%
%
\IEEEauthorblockN{%
    FirstName1 Lastname1\IEEEauthorrefmark{3},\\%
    FirstName2 Lastname2\IEEEauthorrefmark{4}
}%
\IEEEauthorblockA{%
	Chair of Something\\
    Faculty of Amazing Computer Science\\
    University\\
    Optional Address\\
    Email: \{\IEEEauthorrefmark{3}Mail1,\\ \hspace*{1em}\IEEEauthorrefmark{4}Mail2\}@domain.de
}%
}%
%
%








% conference papers do not typically use \thanks and this command
% is locked out in conference mode. If really needed, such as for
% the acknowledgment of grants, issue a \IEEEoverridecommandlockouts
% after \documentclass

% for over three affiliations, or if they all won't fit within the width
% of the page, use this alternative format:
% 
%\author{\IEEEauthorblockN{Michael Shell\IEEEauthorrefmark{1},
%Homer Simpson\IEEEauthorrefmark{2},
%James Kirk\IEEEauthorrefmark{3}, 
%Montgomery Scott\IEEEauthorrefmark{3} and
%Eldon Tyrell\IEEEauthorrefmark{4}}
%\IEEEauthorblockA{\IEEEauthorrefmark{1}School of Electrical and Computer Engineering\\
%Georgia Institute of Technology,
%Atlanta, Georgia 30332--0250\\ Email: see http://www.michaelshell.org/contact.html}
%\IEEEauthorblockA{\IEEEauthorrefmark{2}Twentieth Century Fox, Springfield, USA\\
%Email: homer@thesimpsons.com}
%\IEEEauthorblockA{\IEEEauthorrefmark{3}Starfleet Academy, San Francisco, California 96678-2391\\
%Telephone: (800) 555--1212, Fax: (888) 555--1212}
%\IEEEauthorblockA{\IEEEauthorrefmark{4}Tyrell Inc., 123 Replicant Street, Los Angeles, California 90210--4321}}





==> organization/_templates/IEEE_authors-long.tex <==
% author names and affiliations
% use a multiple column layout for up to three different
% affiliations
\author{%
%
\IEEEauthorblockN{%
    Dennis Krummacker\IEEEauthorrefmark{1}, %
    Christoph Fischer\IEEEauthorrefmark{2}, %
    \\%
    FirstName1 Lastname1\IEEEauthorrefmark{3} and %
    FirstName2 Lastname2\IEEEauthorrefmark{4}%
}%
\IEEEauthorblockA{%
    \IEEEauthorrefmark{1}\IEEEauthorrefmark{2}German Research Center for Artificial Intelligence GmbH (DFKI)%
%     Trippstadter Str. 122\\%
%     67663 Kaiserslautern\\%
	\\%
    \IEEEauthorrefmark{3}Institute1, %
    Some Subtitle 1 %
%     Optional Address, Germany%
    \\%
	\IEEEauthorrefmark{4}Corporation2, %
    Some Subtitle2, %
    Some more Subt2 %
%     Optional Address
    \\%
    Email: %
        \{\IEEEauthorrefmark{1}dennis.krummacker, %
        \IEEEauthorrefmark{2}christoph.fischer\}@dfki.de, %
        \\%
        \IEEEauthorrefmark{3}Mail1@domain1.de, %
        \IEEEauthorrefmark{4}Mail2@domain2.com
}%
}%






% conference papers do not typically use \thanks and this command
% is locked out in conference mode. If really needed, such as for
% the acknowledgment of grants, issue a \IEEEoverridecommandlockouts
% after \documentclass

% for over three affiliations, or if they all won't fit within the width
% of the page, use this alternative format:
% 
%\author{\IEEEauthorblockN{Michael Shell\IEEEauthorrefmark{1},
%Homer Simpson\IEEEauthorrefmark{2},
%James Kirk\IEEEauthorrefmark{3}, 
%Montgomery Scott\IEEEauthorrefmark{3} and
%Eldon Tyrell\IEEEauthorrefmark{4}}
%\IEEEauthorblockA{\IEEEauthorrefmark{1}School of Electrical and Computer Engineering\\
%Georgia Institute of Technology,
%Atlanta, Georgia 30332--0250\\ Email: see http://www.michaelshell.org/contact.html}
%\IEEEauthorblockA{\IEEEauthorrefmark{2}Twentieth Century Fox, Springfield, USA\\
%Email: homer@thesimpsons.com}
%\IEEEauthorblockA{\IEEEauthorrefmark{3}Starfleet Academy, San Francisco, California 96678-2391\\
%Telephone: (800) 555--1212, Fax: (888) 555--1212}
%\IEEEauthorblockA{\IEEEauthorrefmark{4}Tyrell Inc., 123 Replicant Street, Los Angeles, California 90210--4321}}





==> organization/_templates/IEEE_authors.tex <==
% author names and affiliations
% use a multiple column layout for up to three different
% affiliations
\author{%
%
\IEEEauthorblockN{%
    Dennis Krummacker\IEEEauthorrefmark{1},\\%
    Christoph Fischer\IEEEauthorrefmark{2}%
}
\IEEEauthorblockA{%
    German Research Center for\\Artificial Intelligence GmbH, DFKI\\%
    Trippstadter Str. 122\\%
    67663 Kaiserslautern\\%
    Email: %{\tt
      \{%
        \IEEEauthorrefmark{1}dennis.krummacker,\\%
        \hspace*{1em}\IEEEauthorrefmark{2}christoph.fischer%
      \}@dfki.de
    %}%
}
%
\and%
%
\IEEEauthorblockN{%
    FirstName1 Lastname1\IEEEauthorrefmark{3},\\%
    FirstName2 Lastname2\IEEEauthorrefmark{4}
}%
\IEEEauthorblockA{%
	Chair of Something\\
    Faculty of Amazing Computer Science\\
    University\\
    Optional Address\\
    Email: \{\IEEEauthorrefmark{3}Mail1,\\ \hspace*{1em}\IEEEauthorrefmark{4}Mail2\}@domain.de
}%
}%
%
%









%\author{%
%           \IEEEauthorblockN{Michael Shell}
%           \IEEEauthorblockA{School of Electrical and\\Computer Engineering\\
%           Georgia Institute of Technology\\
%           Atlanta, Georgia 30332--0250\\
%           Email: http://www.michaelshell.org/contact.html}
%           \and
%           \IEEEauthorblockN{Homer Simpson}
%           \IEEEauthorblockA{Twentieth Century Fox\\
%           Springfield, USA\\
%           Email: homer@thesimpsons.com}
%           \and
%           \IEEEauthorblockN{James Kirk\\ and Montgomery Scott}
%           \IEEEauthorblockA{Starfleet Academy\\
%           San Francisco, California 96678--2391\\
%           Telephone: (800) 555--1212\\
%           Fax: (888) 555--1212}
%
%}%

% conference papers do not typically use \thanks and this command
% is locked out in conference mode. If really needed, such as for
% the acknowledgment of grants, issue a \IEEEoverridecommandlockouts
% after \documentclass

% for over three affiliations, or if they all won't fit within the width
% of the page, use this alternative format:
% 
%\author{\IEEEauthorblockN{Michael Shell\IEEEauthorrefmark{1},
%Homer Simpson\IEEEauthorrefmark{2},
%James Kirk\IEEEauthorrefmark{3}, 
%Montgomery Scott\IEEEauthorrefmark{3} and
%Eldon Tyrell\IEEEauthorrefmark{4}}
%\IEEEauthorblockA{\IEEEauthorrefmark{1}School of Electrical and Computer Engineering\\
%Georgia Institute of Technology,
%Atlanta, Georgia 30332--0250\\ Email: see http://www.michaelshell.org/contact.html}
%\IEEEauthorblockA{\IEEEauthorrefmark{2}Twentieth Century Fox, Springfield, USA\\
%Email: homer@thesimpsons.com}
%\IEEEauthorblockA{\IEEEauthorrefmark{3}Starfleet Academy, San Francisco, California 96678-2391\\
%Telephone: (800) 555--1212, Fax: (888) 555--1212}
%\IEEEauthorblockA{\IEEEauthorrefmark{4}Tyrell Inc., 123 Replicant Street, Los Angeles, California 90210--4321}}





==> organization/backing/IEEETemplateProvidedExamples.tex <==
% An example of a floating figure using the graphicx package.
% Note that \label must occur AFTER (or within) \caption.
% For figures, \caption should occur after the \includegraphics.
% Note that IEEEtran v1.7 and later has special internal code that
% is designed to preserve the operation of \label within \caption
% even when the captionsoff option is in effect. However, because
% of issues like this, it may be the safest practice to put all your
% \label just after \caption rather than within \caption{}.
%
% Reminder: the "draftcls" or "draftclsnofoot", not "draft", class
% option should be used if it is desired that the figures are to be
% displayed while in draft mode.
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{myfigure}
% where an .eps filename suffix will be assumed under latex, 
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure}

% Note that the IEEE typically puts floats only at the top, even when this
% results in a large percentage of a column being occupied by floats.


% An example of a double column floating figure using two subfigures.
% (The subfig.sty package must be loaded for this to work.)
% The subfigure \label commands are set within each subfloat command,
% and the \label for the overall figure must come after \caption.
% \hfil is used as a separator to get equal spacing.
% Watch out that the combined width of all the subfigures on a 
% line do not exceed the text width or a line break will occur.
%
%\begin{figure*}[!t]
%\centering
%\subfloat[Case I]{\includegraphics[width=2.5in]{box}%
%\label{fig_first_case}}
%\hfil
%\subfloat[Case II]{\includegraphics[width=2.5in]{box}%
%\label{fig_second_case}}
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure*}
%
% Note that often IEEE papers with subfigures do not employ subfigure
% captions (using the optional argument to \subfloat[]), but instead will
% reference/describe all of them (a), (b), etc., within the main caption.
% Be aware that for subfig.sty to generate the (a), (b), etc., subfigure
% labels, the optional argument to \subfloat must be present. If a
% subcaption is not desired, just leave its contents blank,
% e.g., \subfloat[].


% An example of a floating table. Note that, for IEEE style tables, the
% \caption command should come BEFORE the table and, given that table
% captions serve much like titles, are usually capitalized except for words
% such as a, an, and, as, at, but, by, for, in, nor, of, on, or, the, to
% and up, which are usually not capitalized unless they are the first or
% last word of the caption. Table text will default to \footnotesize as
% the IEEE normally uses this smaller font for tables.
% The \label must come after \caption as always.
%
% \begin{table}[!t]
% % increase table row spacing, adjust to taste
% \renewcommand{\arraystretch}{1.3}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
% \caption{An Example of a Table}
% \label{table_example}
% \centering
% % Some packages, such as MDW tools, offer better commands for making tables
% % than the plain LaTeX2e tabular which is used here.
% \begin{tabular}{|c||c|}
% \hline
% One & Two\\
% \hline
% Three & Four\\
% \hline
% \end{tabular}
% \end{table}

==> organization/backing/thebibliography.tex <==
% can use a bibliography generated by BibTeX as a .bbl file
% BibTeX documentation can be easily obtained at:
% http://mirror.ctan.org/biblio/bibtex/contrib/doc/
% The IEEEtran BibTeX style support page is at:
% http://www.michaelshell.org/tex/ieeetran/bibtex/
%\bibliographystyle{IEEEtran}
% argument is your BibTeX string definitions and bibliography database(s)
%\bibliography{IEEEabrv,../bib/paper}
%
% <OR> manually copy in the resultant .bbl file
% set second argument of \begin to the number of references
% (used to reserve space for the reference number labels box)
\begin{thebibliography}{1}

\bibitem{IEEEhowto:kopka}
H.~Kopka and P.~W. Daly, \emph{A Guide to \LaTeX}, 3rd~ed.\hskip 1em plus
  0.5em minus 0.4em\relax Harlow, England: Addison-Wesley, 1999.
  
\bibitem{IEC61158}
, \emph{IEC 61158},

\bibitem{61158-trafficclass}
E DIN EN 61158-1:2017-09 11.4.2

\bibitem{61158-endpoint}
E DIN EN 61158-1:2017-09 9.3.3.3.1

\bibitem{62439-endnode}
DIN EN 62439-1:2010-09 3.1.13

\end{thebibliography}
